Active Dwarf Galaxy Database I: Overlap between active galactic nuclei selected by different techniques

We assemble a sample of 733 dwarf galaxies ($M_{\ast} \le 10^{9.5} \text{M}_\odot$) with signatures of active galactic nuclei (AGN) and explore the intersection between different AGN selection techniques. Objects in our database are compiled from previous studies that identify AGN in dwarf galaxies through spectroscopy, X-ray emission, infrared colors, and optical photometric variability. We apply a uniform set of AGN diagnostic tools to the database using archival data. We find that any single selection method captures no more than half of the overall AGN population, and there is a general disagreement amongst the AGN selection methods in this stellar mass regime. The largest overlap between methods is found when both methods use optical spectroscopic data. In contrast, the populations of AGN intersect the least when comparing those methods that use photometric data at different wavelengths. These results can be used to better constrain the active fraction in dwarf galaxies, which is in turn an important constraint for black hole seed formation models. In a follow-up paper, we will explore links between the effectiveness of each selection technique and host galaxy properties.

==> table_selection_alt.tex <==
% Coloring : 
%   0-24.9  : red \cellcolor[HTML]{fd6666}
%   25-49.9 : orange \cellcolor[HTML]{FAA21A}
%   50-74.9 : yellow \cellcolor[HTML]{FDF07F}
%   75-100 : green \cellcolor[HTML]{44DB5E}
%=================================%

\movetabledown=3.2in
\begin{rotatetable}
\begin{deluxetable}
\centering

\label{tab: summary selection table}

%\textbf{\hspace{1in} Table 3. Overlap between AGN Selection Techniques}

\begin{tabular}{c || c c c c c c c c c c }
\hline

Selection Methods & BPT & [\ion{O}{1}] & [\ion{O}{1}]& [\ion{S}{2}]  & [\ion{S}{2}] & [\ion{He}{2}]  & Broad-line & WISE IR & X-ray & Variability \\
            & (AGN+Comps)& Seyferts    &  LINERS     & Seyferts      & LINERS       & (AGN + Comp)   &               &       &  (AGN) &      \\ 
\hline 
    &  \% & \% & \% & \% & \% & \% & \% & \% & \% & \%   \\
\hline
\begin{tabular}[c]{@{}l@{}}BPT (AGN+Comps)\\ Total: 268\end{tabular} &   -- & \cellcolor[HTML]{FDF07F}58.2 &\cellcolor[HTML]{fd6666} 8.9 & \cellcolor[HTML]{FDF07F}63.4 & \cellcolor[HTML]{fd6666}11.9 & \cellcolor[HTML]{44DB5E}80.2 & \cellcolor[HTML]{fd6666}7.5 & \cellcolor[HTML]{fd6666}12.2 & \cellcolor[HTML]{FDF07F}50.0 & \cellcolor[HTML]{fd6666}13.5 \\[10pt]

\begin{tabular}[c]{@{}l@{}}{[\ion{O}{1}]} Seyferts\\ Total: 270\end{tabular} &  \cellcolor[HTML]{FDF07F}57.7 & -- & \cellcolor[HTML]{fd6666}0.0 & \cellcolor[HTML]{44DB5E}81.4 & \cellcolor[HTML]{fd6666}3.7 & \cellcolor[HTML]{FDF07F}61.4 & \cellcolor[HTML]{fd6666}7.4 & \cellcolor[HTML]{FAA21A}32.9 & \cellcolor[HTML]{FAA21A}38.3 & \cellcolor[HTML]{fd6666}17.5\\[10pt]

\begin{tabular}[c]{@{}l@{}}{[\ion{O}{1}]} LINERS\\ Total: 36\end{tabular} & \cellcolor[HTML]{FDF07F}66.7 & \cellcolor[HTML]{fd6666}0.0 & -- & \cellcolor[HTML]{fd6666}8.3 & \cellcolor[HTML]{FDF07F}69.4 & \cellcolor[HTML]{44DB5E}80.6 & \cellcolor[HTML]{fd6666}2.8 & \cellcolor[HTML]{FAA21A}25.7 & \cellcolor[HTML]{FAA21A}30.0 & \cellcolor[HTML]{FDF07F}55.0\\[10pt]

\begin{tabular}[c]{@{}l@{}}{[\ion{S}{2}]} Seyferts\\ Total: 290\end{tabular} & \cellcolor[HTML]{FDF07F}58.6 & \cellcolor[HTML]{44DB5E}75.8 & \cellcolor[HTML]{fd6666}1.0 & -- & \cellcolor[HTML]{fd6666}0.0 & \cellcolor[HTML]{FDF07F}69.7 & \cellcolor[HTML]{fd6666}5.9 & \cellcolor[HTML]{FAA21A}25.2 & \cellcolor[HTML]{FAA21A}38.8 & \cellcolor[HTML]{fd6666}17.0\\[10pt]

\begin{tabular}[c]{@{}l@{}}{[\ion{S}{2}]} LINERS\\ Total: 61\end{tabular} & \cellcolor[HTML]{FDF07F}52.4 & \cellcolor[HTML]{fd6666}16.4 & \cellcolor[HTML]{FAA21A}41.0 & \cellcolor[HTML]{fd6666}0.0 & -- & \cellcolor[HTML]{44DB5E}82.0 & \cellcolor[HTML]{fd6666}1.6 & \cellcolor[HTML]{fd6666}22.4 & \cellcolor[HTML]{FAA21A}33.3 &\cellcolor[HTML]{FAA21A}42.9 \\[10pt]

\begin{tabular}[c]{@{}l@{}}{[\ion{He}{2}]} (AGN+Comps)\\ Total: 361\end{tabular} & \cellcolor[HTML]{FDF07F}59.5 & \cellcolor[HTML]{FAA21A}46.0 & \cellcolor[HTML]{fd6666}8.0 &\cellcolor[HTML]{FDF07F}56.0 & \cellcolor[HTML]{fd6666}13.8 & -- & \cellcolor[HTML]{fd6666}5.0 & \cellcolor[HTML]{fd6666}14.6 & \cellcolor[HTML]{FAA21A}29.4 & \cellcolor[HTML]{fd6666}20.4 \\[10pt]

\begin{tabular}[c]{@{}l@{}}Broad-line\\ Total: 25\end{tabular} & \cellcolor[HTML]{44DB5E}80.0 & \cellcolor[HTML]{44DB5E}80.0 & \cellcolor[HTML]{fd6666}4.0 &\cellcolor[HTML]{FDF07F}68.0 & \cellcolor[HTML]{fd6666}4.0 &\cellcolor[HTML]{FDF07F}72.0 & -- & \cellcolor[HTML]{FDF07F}62.5 & \cellcolor[HTML]{FDF07F}66.7 & \cellcolor[HTML]{FAA21A}27.3 \\[10pt]

\begin{tabular}[c]{@{}l@{}}WISE IR\\ Total: 201\end{tabular} & \cellcolor[HTML]{fd6666}15.5 & \cellcolor[HTML]{FAA21A}41.5 & \cellcolor[HTML]{fd6666}4.7 & \cellcolor[HTML]{FAA21A}34.2 & \cellcolor[HTML]{fd6666}6.7 & \cellcolor[HTML]{fd6666}24.9 & \cellcolor[HTML]{fd6666}7.8 & -- & \cellcolor[HTML]{fd6666}26.5 & \cellcolor[HTML]{fd6666}16.7\\[10pt]

\begin{tabular}[c]{@{}l@{}}X-ray (AGN)\\ Total: 51\end{tabular} & \cellcolor[HTML]{FDF07F}54.5 & \cellcolor[HTML]{FDF07F}52.2 & \cellcolor[HTML]{fd6666}6.8 & \cellcolor[HTML]{FDF07F}59.1 & \cellcolor[HTML]{fd6666}11.4 & \cellcolor[HTML]{FDF07F}56.8 & \cellcolor[HTML]{fd6666}22.7 & \cellcolor[HTML]{fd6666}25.5 & -- & \cellcolor[HTML]{FAA21A}29.4\\[10pt]

\begin{tabular}[c]{@{}l@{}}Variability\\ Total: 155\end{tabular} & \cellcolor[HTML]{fd6666}17.5 & \cellcolor[HTML]{fd6666}21.2 & \cellcolor[HTML]{fd6666}10.6 & \cellcolor[HTML]{fd6666}22.1 & \cellcolor[HTML]{fd6666}14.4 & \cellcolor[HTML]{FAA21A}35.9 & \cellcolor[HTML]{fd6666}2.9 & \cellcolor[HTML]{fd6666}11.2 & \cellcolor[HTML]{fd6666}14.5 & -- \\[10pt]

\end{tabular}
\end{deluxetable} 
\end{rotatetable}

